Leveraging Natural Language Processing to Augment Structured Social Determinants of Health Data in the Electronic Health Record

Objective: Social determinants of health (SDOH) impact health outcomes and are documented in the electronic health record (EHR) through structured data and unstructured clinical notes. However, clinical notes often contain more comprehensive SDOH information, detailing aspects such as status, severity, and temporality. This work has two primary objectives: i) develop a natural language processing (NLP) information extraction model to capture detailed SDOH information and ii) evaluate the information gain achieved by applying the SDOH extractor to clinical narratives and combining the extracted representations with existing structured data. Materials and Methods: We developed a novel SDOH extractor using a deep learning entity and relation extraction architecture to characterize SDOH across various dimensions. In an EHR case study, we applied the SDOH extractor to a large clinical data set with 225,089 patients and 430,406 notes with social history sections and compared the extracted SDOH information with existing structured data. Results: The SDOH extractor achieved 0.86 F1 on a withheld test set. In the EHR case study, we found extracted SDOH information complements existing structured data with 32% of homeless patients, 19% of current tobacco users, and 10% of drug users only having these health risk factors documented in the clinical narrative. Conclusions: Utilizing EHR data to identify SDOH health risk factors and social needs may improve patient care and outcomes. Semantic representations of text-encoded SDOH information can augment existing structured data, and this more comprehensive SDOH representation can assist health systems in identifying and addressing these social needs.

==> supplemental_files/cover_letter.tex <==
Kevin Lybarger
Assistant Professor
Department of Information Sciences and Technology
George Mason University
4400 University Dr. MSN 1G8
Fairfax, VA 22030
klybarge@gmu.edu 


November 22, 2022 


Dr. Suzanne Bakken
Editor-in-Chief
Journal of the American Medical Informatics Association


Dear Dr. Bakken,

I am pleased to submit an original research article entitled "Leveraging Natural Language Processing to Augment Structured Social Determinants of Health Data in the Electronic Health Record" to be considered for publication in the Journal of the American Medical Informatics Association Focus Issue on Social Determinants of Health (SDOH) Extraction.

This manuscript explores the prevalence of key SDOH information within clinical notes, relative to the available SDOH information in structured data, to quantify the SDOH information gain achievable by leveraging the clinical narrative. We introduce a high-performing deep learning information extraction model for generating structured semantic representations of SDOH from the clinical narrative. We applied the SDOH extraction model to a large data set from the University of Washington with more than 200,000 patients and compared the information available through structured data and text extraction. The results demonstrate that the clinical narrative is extremely important in identifying SDOH risk factors, including tobacco use, drug use, and housing instability. This work advances SDOH information extraction and contributes to our understanding of SDOH information within the electronic health record. 

This manuscript has not been previously published and is not under consideration elsewhere. Dr. Özlem Uzuner, Dr Meliha Yetisgen, and I are co-editors on the JAMIA SDOH focus issue. We have no additional conflicts of interest to disclose. Thank you for your consideration.

Sincerely,

Kevin Lybarger

==> tables/drugs_and_alcohol.tex <==

\def\arraystretch{1.3}
%\begin{tabular}{m{1.7cm} l c c c c c c}
% \toprule
% 
% \textbf{Status} & \textbf{Marijuana} & \textbf{Meth.} & \textbf{Heroin} & \textbf{Cocaine} & \textbf{Opiates} & %\textbf{Oxycodone} & \textbf{Fentanyl} \\
%    \midrule
%    Current   & 2,417 & 1,209 & 369 & 275 & 206 & 13 & 3 \\
%    Past      & 244   & 282   & 120 & 117 & 64  & 8  & 2 \\
%    \bottomrule
%    
%\end{tabular}

\begin{tabular}{m{1.7cm} l l c c}
 \toprule
 \textbf{Category} & \textbf{Type} & \textbf{Current} & \textbf{Past}  \\
    \midrule
    \multirow{13}{*}{Drugs}   & Marijuana        & 2,637 & 298 \\
                             & Methamphetamines & 1,236 & 297 \\
                             & Illicit          & 931   & 122 \\
                             & Heroin           & 635   & 176 \\
                             & Cocaine          & 432   & 174 \\
                             & Recreational     & 402   & 67  \\
                             & Intravenous      & 368   & 78  \\
                             & Opiates          & 221   & 84  \\
                             & Oxycodone        & 20    & 10  \\
                             & Stimulant        & 19    & 6   \\
                             & Fentanyl         & 12    & 5   \\
                             & Percocet         & 11    & 1   \\
                             & LSD              & 5     & 4   \\
    \midrule
    \multirow{11}{*}{Alcohol} & Wine             & 682   & 30  \\
                             & Beer             & 495   & 129 \\
                             & Spirits          & 75    & 0   \\
                             & Liquor           & 68    & 1   \\
                             & Vodka            & 63    & 5   \\
                             & Whiskey          & 28    & 6   \\
                             & Cocktails        & 7     & 0   \\
                             & Scotch           & 6     & 1   \\
                             & Rum              & 5     & 0   \\
                             & Tequila          & 3     & 0   \\
                             & Hard Cider       & 2     & 0   \\
    \bottomrule
    
\end{tabular}

%current	Wine	936	681
%current	Beer	634	455
%current	Vodka	76	57
%current	Whiskey	32	25
%current	Scotch	5	5
%current	Cocktails	9	4
%past	Beer	146	119
%past	Wine	52	28
%past	Vodka	6	5
%past	Whiskey	4	4

%status	grp	cnt	pat_cnt
%current	Marijuana	3307	2417
%current	Methamphetamine	2109	1208
%current	Illicit	676	587
%current	Heroin	542	369
%current	Cocaine	406	275
%current	Intravenous	291	242
%current	Recreational	264	236
%current	Opiates	206	161
%current	Stimulant	17	15
%current	Oxycodone	14	13
%current	Percocet	11	8
%current	LSD	4	4
%current	Hydrocodone	12	4
%current	Fentanyl	7	3
%past	Methamphetamine	384	282
%past	Marijuana	310	244
%past	Heroin	179	120
%past	Cocaine	164	117
%past	Illicit	98	91
%past	Opiates	81	64
%past	Intravenous	75	57
%past	Recreational	46	37
%past	Oxycodone	9	8
%past	Stimulant	2	2
%past	Fentanyl	2	2
%past	Percocet	1	1
%past	LSD	1	1

==> tables/patients_by_sdoh_category.tex <==
\def\arraystretch{1.4}
\begin{center}
\begin{tabular}{l l l l l}
 \toprule
 \textbf{Category} & \textbf{\mbox{Total Patients}} & \textbf{Structured Only} & \textbf{NLP Only} & \textbf{Found in Both} \\
    \hline
    Alcohol & 252,628 & 180,278 (71.3\%) & 21,058 (8.0\%) & 51,292 (20.3\%) \\
    Tobacco & 139,358 & 59,208 (21.4\%) & 50,299 (36.2\%) & 29,851 (42.4\%) \\
    Drug & 204,275 & 132,214 (64.7\%) & 31,785 (15.6\%) & 40,276 (19.7\%) \\
    Employment & 1,573,269 & 1,419,440 (90.2\%) & 30,104 (1.9\%) & 123,725 (7.8\%) \\
    LivingStatus & 11,568 & 7,360 (63.6\%) & 3,692 (31.9\%) & 516 (4.4\%) \\
\end{tabular}
\end{center}

==> tables/shac_counts.tex <==







%TC:ignore 
%\begin{tblr}{llll | l}
\begin{tabular}{llll  l}
\toprule
\textbf{Source} & \textbf{Train}                                    & \textbf{Dev}                        & \textbf{Test}                        & \textbf{Total} \\ \midrule
MIMIC-III       & 1,316   ($\mathcal{D}_{train}^{mimic}$) & 188 ($\mathcal{D}_{dev}^{mimic}$) & 373 ($\mathcal{D}_{test}^{mimic}$) & 1,877 ($\mathcal{D}^{mimic}$)  \\
UW              & 1,751   ($\mathcal{D}_{train}^{uw}   $) & 259 ($\mathcal{D}_{dev}^{uw}   $) & 518 ($\mathcal{D}_{test}^{uw}   $) & 2,528 ($\mathcal{D}^{uw}   $)  \\  \midrule
Total           & 3,067   ($\mathcal{D}_{train}        $) & 447 ($\mathcal{D}_{dev}        $) & 891 ($\mathcal{D}_{test}        $) & 4,405 ($\mathcal{D}$)          \\ \bottomrule
\end{tabular}
%\end{tblr}
%TC:endignore 
